scSSL-Bench: Benchmarking Self-Supervised Learning for Single-Cell Data

Self-supervised learning (SSL) has proven to be a powerful approach for extracting biologically meaningful representations from single-cell data. To advance our understanding of SSL methods applied to single-cell data, we present scSSL-Bench, a comprehensive benchmark that evaluates nineteen SSL methods. Our evaluation spans nine datasets and focuses on three common downstream tasks: batch correction, cell type annotation, and missing modality prediction. Furthermore, we systematically assess various data augmentation strategies. Our analysis reveals task-specific trade-offs: the specialized single-cell frameworks, scVI, CLAIRE, and the finetuned scGPT excel at uni-modal batch correction, while generic SSL methods, such as VICReg and SimCLR, demonstrate superior performance in cell typing and multi-modal data integration. Random masking emerges as the most effective augmentation technique across all tasks, surpassing domain-specific augmentations. Notably, our results indicate the need for a specialized single-cell multi-modal data integration framework. scSSL-Bench provides a standardized evaluation platform and concrete recommendations for applying SSL to single-cell analysis, advancing the convergence of deep learning and single-cell genomics.

==> figures/aug-visualization-new.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.99]{figures/Augmentation-Vsiualization-6.pdf}
    \caption{Overview the CLEAR augmentation pipeline.}
    \label{fig:enter-label}
\end{figure}

==> figures/aug-visualization-old.tex <==
\begin{figure}[h!]
    \centering
    \includesvg[width=\linewidth]{figures/augmentation-overview.svg}
    \caption{Overview of evaluated Augmentations. Our approach differs from that of CLAIRE~\cite{XuhuaRFL23} because it does not discriminate between intra- and inter-batch nearest neighbors.}
    \label{fig:enter-label}
\end{figure}

==> figures/downstream/missing_modality.tex <==
\begin{figure}[!t]
    \centering
    % \input{figures/downstream/missing_modality}
    
    % \vspace{-0.4cm}
    \caption{Missing Modality Prediction}
    \label{fig:TaskMissingModality}
\end{figure}

==> tables/bc_ours.tex <==
\begin{table}[htp!]
\centering
\caption{Bio conservation, batch correction and total for OUR pipeline}
\resizebox{\linewidth}{!}{
\setlength\tabcolsep{1.8pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{HIC}} & \multicolumn{3}{c|}{\textbf{MCA}} & \multicolumn{3}{c|}{\textbf{PBMC}} & \multicolumn{3}{c|}{\textbf{Lung}} & \multicolumn{3}{c}{\textbf{Pancreas}} \\
& Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total \\
\midrule
\multirow{2}{*}{SimCLR} & 0.837 & 0.552 & 0.723 & 0.777 & 0.307 & 0.589 & 0.837 & 0.544 & 0.72 & 0.194 & 0.375 & 0.266 & 0.707 & 0.281 & 0.536 \\
& \pmS{0.026} & \pmS{0.028} & \pmS{0.019} & \pmS{0.041} & \pmS{0.03} & \pmS{0.03} & \pmS{0.026} & \pmS{0.027} & \pmS{0.019} & \pmS{0.01} & \pmS{0.012} & \pmS{0.008} & \pmS{0.05} & \pmS{0.036} & \pmS{0.035} \\
\multirow{2}{*}{MoCo} & 0.764 & 0.524 & 0.668 & 0.27 & 0.407 & 0.325 & 0.251 & 0.445 & 0.329 & 0.22 & 0.432 & 0.305 & 0.691 & 0.446 & 0.593 \\
& \pmS{0.021} & \pmS{0.016} & \pmS{0.018} & \pmS{0.023} & \pmS{0.021} & \pmS{0.01} & \pmS{0.011} & \pmS{0.009} & \pmS{0.01} & \pmS{0.004} & \pmS{0.011} & \pmS{0.004} & \pmS{0.018} & \pmS{0.026} & \pmS{0.016} \\
\multirow{2}{*}{SimSiam} & 0.696 & 0.634 & 0.671 & 0.593 & 0.374 & 0.505 & 0.696 & 0.618 & 0.665 & 0.853 & 0.553 & 0.733 & 0.356 & 0.436 & 0.388 \\
& \pmS{0.044} & \pmS{0.044} & \pmS{0.02} & \pmS{0.063} & \pmS{0.038} & \pmS{0.042} & \pmS{0.044} & \pmS{0.043} & \pmS{0.022} & \pmS{0.053} & \pmS{0.032} & \pmS{0.023} & \pmS{0.108} & \pmS{0.049} & \pmS{0.06} \\
\multirow{2}{*}{NNCLR} & 0.742 & 0.59 & 0.681 & 0.652 & 0.326 & 0.522 & 0.742 & 0.579 & 0.677 & 0.166 & 0.419 & 0.267 & 0.474 & 0.327 & 0.415 \\
& \pmS{0.019} & \pmS{0.04} & \pmS{0.023} & \pmS{0.027} & \pmS{0.046} & \pmS{0.032} & \pmS{0.019} & \pmS{0.039} & \pmS{0.023} & \pmS{0.015} & \pmS{0.012} & \pmS{0.008} & \pmS{0.044} & \pmS{0.055} & \pmS{0.045} \\
\multirow{2}{*}{BYOL} & 0.72 & 0.752 & 0.733 & 0.622 & 0.515 & 0.579 & 0.72 & 0.735 & 0.726 & 0.122 & 0.609 & 0.317 & 0.411 & 0.618 & 0.494 \\
& \pmS{0.036} & \pmS{0.033} & \pmS{0.01} & \pmS{0.048} & \pmS{0.028} & \pmS{0.02} & \pmS{0.036} & \pmS{0.032} & \pmS{0.01} & \pmS{0.012} & \pmS{0.021} & \pmS{0.008} & \pmS{0.089} & \pmS{0.042} & \pmS{0.039} \\
\multirow{2}{*}{VICReg} & 0.916 & 0.578 & 0.781 & 0.89 & 0.382 & 0.686 & 0.916 & 0.576 & 0.78 & 0.488 & 0.512 & 0.498 & 0.873 & 0.329 & 0.656 \\
& \pmS{0.014} & \pmS{0.023} & \pmS{0.011} & \pmS{0.019} & \pmS{0.029} & \pmS{0.017} & \pmS{0.014} & \pmS{0.023} & \pmS{0.011} & \pmS{0.023} & \pmS{0.019} & \pmS{0.018} & \pmS{0.02} & \pmS{0.035} & \pmS{0.019} \\
Barlow & 0.072 & 0.453 & 0.225 & 0.66 & 0.3 & 0.516 & 0.072 & 0.432 & 0.216 & 0.347 & 0.417 & 0.375 & 0.5 & 0.28 & 0.412 \\
Twins & \pmS{0.006} & \pmS{0.008} & \pmS{0.005} & \pmS{0.012} & \pmS{0.04} & \pmS{0.011} & \pmS{0.006} & \pmS{0.008} & \pmS{0.005} & \pmS{0.017} & \pmS{0.016} & \pmS{0.01} & \pmS{0.029} & \pmS{0.054} & \pmS{0.009} \\
\bottomrule
\end{tabular}
}
\label{tab:ours_bc}
\end{table}


==> tables/model-table-1.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ll}
\toprule
\textbf{Representation Dimension} & All Models\\
\textbf{Projector Upscaling Factor} & BarlowTwins, VICReg, BYOL\\
\textbf{Projector Downscaling Factor} & NNCLR, SimSiam\\
\bottomrule
\\
\end{tabular}
\caption{\textbf{\textcolor{red}{Remove this table @ submission?}}}
\label{tab:options}
\end{table}


==> tables/table_template_bc.tex <==
\begin{table}[t!]
\centering
\caption{Bio Conservation, Batch Correction and Total Score for the CLEAR Pipeline}
\resizebox{\linewidth}{!}{
\setlength\tabcolsep{1.8pt}
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{HIC}} & \multicolumn{3}{c|}{\textbf{MCA}} & \multicolumn{3}{c|}{\textbf{PBMC}} & \multicolumn{3}{c|}{\textbf{Lung}} & \multicolumn{3}{c}{\textbf{Pancreas}} \\
& Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total & Bio & Batch & Total \\
\midrule
\multirow{2}{*}{SimCLR} & \textbf{0.939} & 0.383 & \textbf{0.717} & \textbf{0.961} & 0.351 & \textbf{0.717} & \textbf{0.962} & 0.456 & \textbf{0.76} & \textbf{0.966} & 0.508 & \textbf{0.783} & \textbf{0.955} & 0.367 & \textbf{0.72} \\
                        & \pmS{0.018} & \pmS{0.02} & \pmS{0.015} & \pmS{0.017} & \pmS{0.024} & \pmS{0.015} & \pmS{0.017} & \pmS{0.013} & \pmS{0.012} & \pmS{0.015} & \pmS{0.009} & \pmS{0.01} & \pmS{0.021} & \pmS{0.024} & \pmS{0.017} \\
\multirow{2}{*}{MoCo}   & 0.756 & 0.535 & 0.668 & 0.292 & \textbf{0.59} & 0.411 & 0.242 & 0.371 & 0.294 & 0.098 & 0.486 & 0.253 & 0.74 & 0.566 & 0.67 \\
                        & \pmS{0.014} & \pmS{0.016} & \pmS{0.01} & \pmS{0.035} & \pmS{0.041} & \pmS{0.021} & \pmS{0.01} & \pmS{0.022} & \pmS{0.014} & \pmS{0.006} & \pmS{0.02} & \pmS{0.008} & \pmS{0.038} & \pmS{0.074} & \pmS{0.016} \\
\multirow{2}{*}{SimSiam}& 0.614 & 0.397 & 0.527 & 0.657 & 0.332 & 0.527 & 0.671 & 0.463 & 0.588 & 0.696 & 0.523 & 0.627 & 0.563 & 0.391 & 0.494 \\
                        & \pmS{0.029} & \pmS{0.058} & \pmS{0.027} & \pmS{0.034} & \pmS{0.058} & \pmS{0.029} & \pmS{0.034} & \pmS{0.051} & \pmS{0.025} & \pmS{0.028} & \pmS{0.057} & \pmS{0.022} & \pmS{0.034} & \pmS{0.075} & \pmS{0.034} \\
\multirow{2}{*}{NNCLR}  & 0.766 & 0.362 & 0.604 & 0.793 & 0.315 & 0.602 & 0.8 & 0.426 & 0.65 & 0.816 & 0.47 & 0.677 & 0.744 & 0.329 & 0.578 \\
                        & \pmS{0.053} & \pmS{0.019} & \pmS{0.037} & \pmS{0.051} & \pmS{0.019} & \pmS{0.037} & \pmS{0.049} & \pmS{0.013} & \pmS{0.032} & \pmS{0.046} & \pmS{0.016} & \pmS{0.028} & \pmS{0.064} & \pmS{0.026} & \pmS{0.046} \\
\multirow{2}{*}{BYOL}   & 0.59 & \textbf{0.57} & 0.582 & 0.643 & 0.494 & 0.584 & 0.656 & \textbf{0.604} & 0.635 & 0.682 & \textbf{0.661} & 0.674 & 0.528 & \textbf{0.607} & 0.56 \\
                        & \pmS{0.034} & \pmS{0.017} & \pmS{0.023} & \pmS{0.022} & \pmS{0.029} & \pmS{0.021} & \pmS{0.021} & \pmS{0.015} & \pmS{0.015} & \pmS{0.019} & \pmS{0.014} & \pmS{0.013} & \pmS{0.042} & \pmS{0.038} & \pmS{0.034} \\
\multirow{2}{*}{VICReg} & 0.914 & 0.418 & 0.715 & 0.931 & 0.397 & \textbf{0.717} & 0.931 & 0.472 & 0.748 & 0.935 & 0.509 & 0.765 & 0.919 & 0.418 & 0.719 \\
                        & \pmS{0.013} & \pmS{0.016} & \pmS{0.004} & \pmS{0.014} & \pmS{0.017} & \pmS{0.003} & \pmS{0.013} & \pmS{0.011} & \pmS{0.006} & \pmS{0.011} & \pmS{0.011} & \pmS{0.007} & \pmS{0.014} & \pmS{0.021} & \pmS{0.006} \\
Barlow                  & 0.881 & 0.374 & 0.678 & 0.908 & 0.352 & 0.686 & 0.912 & 0.427 & 0.718 & 0.919 & 0.46 & 0.735 & 0.884 & 0.376 & 0.681 \\
Twins                   & \pmS{0.037} & \pmS{0.032} & \pmS{0.028} & \pmS{0.038} & \pmS{0.036} & \pmS{0.029} & \pmS{0.037} & \pmS{0.025} & \pmS{0.027} & \pmS{0.036} & \pmS{0.026} & \pmS{0.026} & \pmS{0.047} & \pmS{0.054} & \pmS{0.04} \\
\multirow{2}{*}{Concerto} & & & & & & & & & & & & & & & \\
& & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
}
\label{tab:clear_bc}
\end{table}
